Dark matter mass loss in galaxy flybys: dependence on impact parameter

Galaxy flybys, interactions where two independent halos inter-penetrate but detach at a later time and do not merge, occur frequently at lower redshifts. These interactions can significantly impact the evolution of individual galaxies - from the mass loss and shape transformation to the emergence of tidal features and formation of morphological disc structures. The main focus of this paper is on the dark matter mass loss of the secondary, intruder galaxy, with the goal of determining a functional relationship between the impact parameter and dark matter mass loss. Series of N-body simulations of typical galaxy flybys (10:1 mass ratio) with differing impact parameters show that the dark matter halo leftover mass of the intruder galaxy follows a logarithmic growth law with impact parameter, regardless of the way the total halo mass is estimated. The lost mass then, clearly, follows the exponential decay law. The stellar component stretches faster as the impact parameter decreases, following the exponential decay law with impact parameter. Functional dependence on impact parameter in all cases seems universal, but the fitting parameters are likely sensitive to the interaction parameters and initial conditions (e.g. the mass ratio of interacting galaxies, initial relative velocity of the intruder galaxy, interaction duration). While typical flybys, investigated here, could not be the sole culprit behind the formation of ultra-diffuse or dark matter deficient galaxies, they can still contribute significantly. Rare, atypical and stronger flybys are worth further exploring.

==> DARK MATTER MASS LOSS IN GALAXY FLYBYS/abr_saj.tex <==
\newcommand\aap{A\&A}%     % Astronomy and Astrophysics 
\newcommand\aapr{A\&ARv}%  % Astronomy and Astrophysics Reviews 
\newcommand\aaps{A\&AS}%    % Astronomy and Astrophysics, Supplement 
\newcommand\aas{AAS Meeting Abstracts}% American Astronomical Society Meeting 
%Abstracts
\newcommand\actaa{AcA}%  % Acta Astronomica
\newcommand\aj{AJ}%        % Astronomical Journal 
\newcommand\ao{ApOpt}%   % Applied Optics ++
\newcommand\apj{ApJ}%    % Astrophysical Journal ++
\newcommand\apjl{ApJL}     % Astrophysical Journal, Letters 
\newcommand\apjs{ApJS}%    % Astrophysical Journal, Supplement 
\newcommand\aplett{Astrophys.~Lett.}%  % Astrophysics Letters 
\newcommand\apspr{Astrophys.~Space~Phys.~Res.}% % Astrophysics Space Physics 
%Research 
\newcommand\apss{Ap\&SS}%  % Astrophysics and Space Science 
\newcommand\araa{ARA\&A}%  % Annual Review of Astron and Astrophys 
\newcommand\azh{AZh}%       % Astronomicheskii Zhurnal 
\newcommand\baas{BAAS}%     % Bulletin of the AAS 
\newcommand\bac{Bull. astr. Inst. Czechosl.}
\newcommand\bain{BAN}% % Bulletin Astronomical Institute of the Netherlands 
\newcommand\caa{ChA\&A}%  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{ChJA\&A}%  % Chinese Journal of Astronomy and Astrophysics
\newcommand\dps{AAS/DPS Meeting Abstracts}% American Astronomical 
%Society/Division for Planetary Sciences Meeting Abstracts
\newcommand\fcp{FCPh}%   % Fundamental Cosmic Physics 
\newcommand\gca{GeoCoA}% % Geochimica Cosmochimica Acta 
\newcommand\grl{Geophys.~Res.~Lett.}%  % Geophysics Research Letters 
\newcommand\iaucirc{IAUC}% % IAU Cirulars 
\newcommand\icarus{Icar}% % Icarus
\newcommand\jcap{JCAP}%  % Journal of Cosmology and Astroparticle Physics
\newcommand\jcp{JChPh}%     % Journal of Chemical Physics 
\newcommand\jgr{JGR}%     % Journal of Geophysics Research 
\newcommand\jqsrt{JQSRT}%   % Journal of Quantitiative Spectroscopy and 
%Radiative Trasfer 
\newcommand\jrasc{JRASC}%   % Journal of the RAS of Canada 
\newcommand\maps{M\&PS}% Meteoritics and Planetary Science
\newcommand\memras{MmRAS}%  % Memoirs of the RAS 
\newcommand\memsai{MmSAI}% % Mem. Societa Astronomica Italiana 
\newcommand\mnras{MNRAS}%   % Monthly Notices of the RAS 
\newcommand\na{NewA}%  % New Astronomy
\newcommand\nar{NewAR}%  % New Astronomy Review
\newcommand\nat{Natur}%  % Nature 
\newcommand\nphysa{NuPhA}%     % Nuclear Physics A 
\newcommand\pasa{PASA}%  % Publications of the Astron. Soc. of Australia
\newcommand\pasj{PASJ}%     % Publications of the ASJ 
\newcommand\pasp{PASP}%     % Publications of the ASP 
\newcommand\physrep{PhR}%       % Physics Reports 
\newcommand\physscr{PhyS}%        % Physica Scripta 
\newcommand\planss{Planet.~Space~Sci.}%  % Planetary Space Science 
\newcommand\pra{PhRvA}% % Physical Review A: General Physics ++
\newcommand\prb{PhRvB}% % Physical Review B: Solid State ++
\newcommand\prc{PhRvC}% % Physical Review C ++
\newcommand\prd{PhRvD}% % Physical Review D ++
\newcommand\pre{PhRvE}% % Physical Review E ++
\newcommand\prl{PhRvL}% % Physical Review Letters 
\newcommand\procspie{Proc.~SPIE}%      % Proceedings of the SPIE 
\newcommand\qjras{QJRAS}%   % Quarterly Journal of the RAS 
\newcommand\rmxaa{RMxAA}%  % Revista Mexicana de Astronomia y Astrofisica
\newcommand\skytel{S\&T}%   % Sky and Telescope 
\newcommand\solphys{SoPh}% % Solar Physics 
\newcommand\sovast{Soviet~Ast.}% % Soviet Astronomy 
\newcommand\ssr{SSRv}% % Space Science Reviews 
\newcommand\zap{ZA}%       % Zeitschrift fuer Astrophysik 

\let\astap=\aap 
\let\apjlett=\apjl 
\let\apjsupp=\apjs 
\let\applopt=\ao 





==> DARK MATTER MASS LOSS IN GALAXY FLYBYS/astro.tex <==
\def\tg{\mathop{\rm tg}\nolimits}
\def\arctg{\mathop{\rm arctg}\nolimits}

\def\point#1{\hbox{\setbox7=\hbox to0.6em{\hfil.\hfil}%
\setbox8=\hbox to0.5em{\hfil$^{#1}$\hfil}%
\box7\kern-0.5em\box8}}

\def\dan{\point{\rm d}}
\def\cas{\point{\rm h}}
\def\minut{\point{\rm m}}
\def\sekund{\point{\mathrm{s}}}

\def\oo{\point{\circ}}
\def\lll{\point{\prime}}
\def\uu{\point{\prime\prime}}




==> DARK MATTER MASS LOSS IN GALAXY FLYBYS/mjyu.tex <==
\def\nava{\leavevmode\hbox{,\kern-0.09em,}}%yu-navodnik-pocetni
\def\navb{\char'134}                                      %yu-navodnik-krajnji
\def\DJ{\leavevmode\setbox0=\hbox{D}\kern0pt
 \rlap{\kern.04em\raise.188\ht0\hbox{-}}D}
\def\dj{\leavevmode\setbox0=\hbox{d}\kern0pt
 \rlap{\kern.215em\raise.46\ht0\hbox{-}}d}
\def\SH{\v S} \def\sh{\v s} % Sasinci
\def\CJ{\' C} \def\cj{\' c} % Cicevac
\def\CH{\v C} \def\ch{\v c} % Xaxak
\def\Z{\v Z} \def\z{\v z} % Zuzemberk
\def\br{\break}



==> DARK MATTER MASS LOSS IN GALAXY FLYBYS/wncyr.tex <==
\def\rrmd{\font\tipo=wncyr12\tip}%
\def\rbfd{\font\tipo=wncyb12\tip}%
\def\rssd{\font\tipo=wncyss12\tip}%
\def\rrm{\font\tipo=wncyr10\tip}%
\def\rbf{\font\tipo=wncyb10\tip}%
\def\rit{\font\tipo=wncyi10\tip}%
\def\rss{\font\tipo=wncyss10\tip}%
\def\rsc{\font\tipo=wncysc10\tip}%
\def\rrmdev{\font\tipo=wncyr9\tip}%
\def\rbfdev{\font\tipo=wncyb9\tip}%
\def\ritdev{\font\tipo=wncyi9\tip}%
\def\rssdev{\font\tipo=wncyss9\tip}%
\def\rrmos{\font\tipo=wncyr8\tip}%
\def\rbfos{\font\tipo=wncyb8\tip}%
\def\ritos{\font\tipo=wncyi8\tip}%
\def\rssos{\font\tipo=wncyss8\tip}%
\def\rrmsev{\font\tipo=wncyr7\tip}%
\def\rbfsev{\font\tipo=wncyb7\tip}%
\def\ritsev{\font\tipo=wncyi7\tip}%
\def\tip{\relax\tipo\def\DD{\tipo\char'006}\def\dd{\tipo\char'016}% \tip
\def\DJ{\DD}\def\dj{\dd}% 
\def\ZZ{\tipo\char'021}\def\zz{\tipo\char'031}%
\def\Z{\ZZ}\def\z{\zz}%
\def\LJ{\tipo\char'001}\def\lj{\tipo\char'011}%
\def\NJ{\tipo\char'000}\def\nj{\tipo\char'010}%
\def\CC{\tipo\char'007}\def\cc{\tipo\char'017}%
\def\DZ{\tipo\char'002}\def\dz{\tipo\char'012}%
\def\XX{Q}\def\xx{q}%
\def\JJ{J}\def\jj{j}% 
\def\SS{X}\def\ss{x}%
\def\JA{\tipo\char'027}\def\ja{\tipo\char'037}%
\def\SC{W}\def\sc{w}%
\def\CJ{\CC}\def\cj{\cc}%
\def\CH{Q}\def\ch{q}%
\def\SH{X}\def\sh{x}%
% sch="x"; tvrdo i = "y"; ja = "j"; schtsch = "w"; tsch = "q"
\def\EE{\tipo\char'003}\def\ee{\tipo\char'013}% "e oborotnoe"
\def\JI{\tipo\char'022}\def\ji{\tipo\char'032}% rusko "j"
\def\JU{\tipo\char'020}\def\ju{\tipo\char'030}%
\def\M{\tipo\char'136}\def\m{\tipo\char'176}% meki znak
\def\TV{\tipo\char'137}\def\tv{\tipo\char'177}% tvrdi znak
\def\rnava{\tipo\char'074}\def\rnavb{\tipo\char'076}% ruski navodnici
\def\snava{\leavevmode\hbox{,\kern-0.06em,}}% yu-
\def\snavb{\tipo\char'134}}% navodnici
\def\br{\break}%




==> abr_saj.tex <==
\newcommand\aap{A\&A}%     % Astronomy and Astrophysics 
\newcommand\aapr{A\&ARv}%  % Astronomy and Astrophysics Reviews 
\newcommand\aaps{A\&AS}%    % Astronomy and Astrophysics, Supplement 
\newcommand\aas{AAS Meeting Abstracts}% American Astronomical Society Meeting 
%Abstracts
\newcommand\actaa{AcA}%  % Acta Astronomica
\newcommand\aj{AJ}%        % Astronomical Journal 
\newcommand\ao{ApOpt}%   % Applied Optics ++
\newcommand\apj{ApJ}%    % Astrophysical Journal ++
\newcommand\apjl{ApJL}     % Astrophysical Journal, Letters 
\newcommand\apjs{ApJS}%    % Astrophysical Journal, Supplement 
\newcommand\aplett{Astrophys.~Lett.}%  % Astrophysics Letters 
\newcommand\apspr{Astrophys.~Space~Phys.~Res.}% % Astrophysics Space Physics 
%Research 
\newcommand\apss{Ap\&SS}%  % Astrophysics and Space Science 
\newcommand\araa{ARA\&A}%  % Annual Review of Astron and Astrophys 
\newcommand\azh{AZh}%       % Astronomicheskii Zhurnal 
\newcommand\baas{BAAS}%     % Bulletin of the AAS 
\newcommand\bac{Bull. astr. Inst. Czechosl.}
\newcommand\bain{BAN}% % Bulletin Astronomical Institute of the Netherlands 
\newcommand\caa{ChA\&A}%  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{ChJA\&A}%  % Chinese Journal of Astronomy and Astrophysics
\newcommand\dps{AAS/DPS Meeting Abstracts}% American Astronomical 
%Society/Division for Planetary Sciences Meeting Abstracts
\newcommand\fcp{FCPh}%   % Fundamental Cosmic Physics 
\newcommand\gca{GeoCoA}% % Geochimica Cosmochimica Acta 
\newcommand\grl{Geophys.~Res.~Lett.}%  % Geophysics Research Letters 
\newcommand\iaucirc{IAUC}% % IAU Cirulars 
\newcommand\icarus{Icar}% % Icarus
\newcommand\jcap{JCAP}%  % Journal of Cosmology and Astroparticle Physics
\newcommand\jcp{JChPh}%     % Journal of Chemical Physics 
\newcommand\jgr{JGR}%     % Journal of Geophysics Research 
\newcommand\jqsrt{JQSRT}%   % Journal of Quantitiative Spectroscopy and 
%Radiative Trasfer 
\newcommand\jrasc{JRASC}%   % Journal of the RAS of Canada 
\newcommand\maps{M\&PS}% Meteoritics and Planetary Science
\newcommand\memras{MmRAS}%  % Memoirs of the RAS 
\newcommand\memsai{MmSAI}% % Mem. Societa Astronomica Italiana 
\newcommand\mnras{MNRAS}%   % Monthly Notices of the RAS 
\newcommand\na{NewA}%  % New Astronomy
\newcommand\nar{NewAR}%  % New Astronomy Review
\newcommand\nat{Natur}%  % Nature 
\newcommand\nphysa{NuPhA}%     % Nuclear Physics A 
\newcommand\pasa{PASA}%  % Publications of the Astron. Soc. of Australia
\newcommand\pasj{PASJ}%     % Publications of the ASJ 
\newcommand\pasp{PASP}%     % Publications of the ASP 
\newcommand\physrep{PhR}%       % Physics Reports 
\newcommand\physscr{PhyS}%        % Physica Scripta 
\newcommand\planss{Planet.~Space~Sci.}%  % Planetary Space Science 
\newcommand\pra{PhRvA}% % Physical Review A: General Physics ++
\newcommand\prb{PhRvB}% % Physical Review B: Solid State ++
\newcommand\prc{PhRvC}% % Physical Review C ++
\newcommand\prd{PhRvD}% % Physical Review D ++
\newcommand\pre{PhRvE}% % Physical Review E ++
\newcommand\prl{PhRvL}% % Physical Review Letters 
\newcommand\procspie{Proc.~SPIE}%      % Proceedings of the SPIE 
\newcommand\qjras{QJRAS}%   % Quarterly Journal of the RAS 
\newcommand\rmxaa{RMxAA}%  % Revista Mexicana de Astronomia y Astrofisica
\newcommand\skytel{S\&T}%   % Sky and Telescope 
\newcommand\solphys{SoPh}% % Solar Physics 
\newcommand\sovast{Soviet~Ast.}% % Soviet Astronomy 
\newcommand\ssr{SSRv}% % Space Science Reviews 
\newcommand\zap{ZA}%       % Zeitschrift fuer Astrophysik 

\let\astap=\aap 
\let\apjlett=\apjl 
\let\apjsupp=\apjs 
\let\applopt=\ao 





==> astro.tex <==
\def\tg{\mathop{\rm tg}\nolimits}
\def\arctg{\mathop{\rm arctg}\nolimits}

\def\point#1{\hbox{\setbox7=\hbox to0.6em{\hfil.\hfil}%
\setbox8=\hbox to0.5em{\hfil$^{#1}$\hfil}%
\box7\kern-0.5em\box8}}

\def\dan{\point{\rm d}}
\def\cas{\point{\rm h}}
\def\minut{\point{\rm m}}
\def\sekund{\point{\mathrm{s}}}

\def\oo{\point{\circ}}
\def\lll{\point{\prime}}
\def\uu{\point{\prime\prime}}




==> mjyu.tex <==
\def\nava{\leavevmode\hbox{,\kern-0.09em,}}%yu-navodnik-pocetni
\def\navb{\char'134}                                      %yu-navodnik-krajnji
\def\DJ{\leavevmode\setbox0=\hbox{D}\kern0pt
 \rlap{\kern.04em\raise.188\ht0\hbox{-}}D}
\def\dj{\leavevmode\setbox0=\hbox{d}\kern0pt
 \rlap{\kern.215em\raise.46\ht0\hbox{-}}d}
\def\SH{\v S} \def\sh{\v s} % Sasinci
\def\CJ{\' C} \def\cj{\' c} % Cicevac
\def\CH{\v C} \def\ch{\v c} % Xaxak
\def\Z{\v Z} \def\z{\v z} % Zuzemberk
\def\br{\break}



==> wncyr.tex <==
\def\rrmd{\font\tipo=wncyr12\tip}%
\def\rbfd{\font\tipo=wncyb12\tip}%
\def\rssd{\font\tipo=wncyss12\tip}%
\def\rrm{\font\tipo=wncyr10\tip}%
\def\rbf{\font\tipo=wncyb10\tip}%
\def\rit{\font\tipo=wncyi10\tip}%
\def\rss{\font\tipo=wncyss10\tip}%
\def\rsc{\font\tipo=wncysc10\tip}%
\def\rrmdev{\font\tipo=wncyr9\tip}%
\def\rbfdev{\font\tipo=wncyb9\tip}%
\def\ritdev{\font\tipo=wncyi9\tip}%
\def\rssdev{\font\tipo=wncyss9\tip}%
\def\rrmos{\font\tipo=wncyr8\tip}%
\def\rbfos{\font\tipo=wncyb8\tip}%
\def\ritos{\font\tipo=wncyi8\tip}%
\def\rssos{\font\tipo=wncyss8\tip}%
\def\rrmsev{\font\tipo=wncyr7\tip}%
\def\rbfsev{\font\tipo=wncyb7\tip}%
\def\ritsev{\font\tipo=wncyi7\tip}%
\def\tip{\relax\tipo\def\DD{\tipo\char'006}\def\dd{\tipo\char'016}% \tip
\def\DJ{\DD}\def\dj{\dd}% 
\def\ZZ{\tipo\char'021}\def\zz{\tipo\char'031}%
\def\Z{\ZZ}\def\z{\zz}%
\def\LJ{\tipo\char'001}\def\lj{\tipo\char'011}%
\def\NJ{\tipo\char'000}\def\nj{\tipo\char'010}%
\def\CC{\tipo\char'007}\def\cc{\tipo\char'017}%
\def\DZ{\tipo\char'002}\def\dz{\tipo\char'012}%
\def\XX{Q}\def\xx{q}%
\def\JJ{J}\def\jj{j}% 
\def\SS{X}\def\ss{x}%
\def\JA{\tipo\char'027}\def\ja{\tipo\char'037}%
\def\SC{W}\def\sc{w}%
\def\CJ{\CC}\def\cj{\cc}%
\def\CH{Q}\def\ch{q}%
\def\SH{X}\def\sh{x}%
% sch="x"; tvrdo i = "y"; ja = "j"; schtsch = "w"; tsch = "q"
\def\EE{\tipo\char'003}\def\ee{\tipo\char'013}% "e oborotnoe"
\def\JI{\tipo\char'022}\def\ji{\tipo\char'032}% rusko "j"
\def\JU{\tipo\char'020}\def\ju{\tipo\char'030}%
\def\M{\tipo\char'136}\def\m{\tipo\char'176}% meki znak
\def\TV{\tipo\char'137}\def\tv{\tipo\char'177}% tvrdi znak
\def\rnava{\tipo\char'074}\def\rnavb{\tipo\char'076}% ruski navodnici
\def\snava{\leavevmode\hbox{,\kern-0.06em,}}% yu-
\def\snavb{\tipo\char'134}}% navodnici
\def\br{\break}%



